Weighted First Order Model Counting with Directed Acyclic Graph Axioms

Statistical Relational Learning (SRL) integrates First-Order Logic (FOL) and probability theory for learning and inference over relational data. Probabilistic inference and learning in many SRL models can be reduced to Weighted First Order Model Counting (WFOMC). However, WFOMC is known to be intractable ($\mathrm{\#P_1-}$ complete). Hence, logical fragments that admit polynomial time WFOMC are of significant interest. Such fragments are called domain liftable. Recent line of works have shown the two-variable fragment of FOL, extended with counting quantifiers ($\mathrm{C^2}$) to be domain-liftable. However, many properties of real-world data can not be modelled in $\mathrm{C^2}$. In fact many ubiquitous properties of real-world data are inexressible in FOL. Acyclicity is one such property, found in citation networks, genealogy data, temporal data e.t.c. In this paper we aim to address this problem by investigating the domain liftability of directed acyclicity constraints. We show that the fragment $\mathrm{C^2}$ with a Directed Acyclic Graph (DAG) axiom, i.e., a predicate in the language is axiomatized to represent a DAG, is domain-liftable. We present a method based on principle of inclusion-exclusion for WFOMC of $\mathrm{C^2}$ formulas extended with DAG axioms.

==> 02_related.tex <==
\section{Related Work}
WFOMC was initially formalised in \cite{LIFTED_PI_KB_COMPLETION, PTP}. 
The paper generalizes \emph{knowledge compilation} techniques to FOL theories, providing  an algorithm for Symmetric-WFOMC over universally quantified FOL theories. \cite{DOMAIN_RECURSION} introduced the notion of domain lifted theories, also demonstrating that a theory composed of a set of universally quantified clauses containing at most two variables is domain liftable. In \cite{broeck2013}, these results are extended to full FO$^2$  (i.e. where existential quantification is allowed) by introducing a  skolemization procedure for WFOMC.  \cite{Symmetric_Weighted} provides a uniform complexity theoretic analysis of Symmetric-WFOMC, providing a closed-form formula for WFOMC in the universally quantified fragment of FO$^2$. They also show that in the three variable fragment of FOL, there is a formula whose WFOMC cannot be computed in polynomial time, demonstrating that WFOMC is $\#P_1-$complete in general. In \cite{kuusisto2018weighted}, domain liftability results are extended to FO$^2$ with a functionality axiom, and for sentences in \emph{uniform one-dimensional fragment} U$_1$ \cite{kieronski2015uniform}. It also proposes a closed-form formula for WFOMC in $\mathrm{FO^{2}}$ with functionality constraints. \cite{kuzelka2020weighted} recently proposed a uniform treatment of WFOMC for FO$^2$ with cardinality constraints  and counting quantifiers, proving these theories to be domain-liftable. \cite{AAAI_Sagar} on the other hand provide a more analytical approach to dealing with WFOMC in C$^2$ and expand this fragment with a more expressive class of weight functions than symmetric weight functions. Furthermore, they show that this class of weight functions is atleast as expressive as complex valued weight functions introduced in \cite{complexMLNkuzelka2020}.  



Recent results have focused on expanding the expressivity of C$^2$ with additional constraints like the linear order axiom \cite{LinearOrder} and tree axiom \cite{Tree}.  The approaches proposed in this paper are most closely related to \cite{Symmetric_Weighted}, \cite{kuzelka2020weighted} and  \cite{LinearOrder}. As we begin with the formula proposed in \cite{Symmetric_Weighted} for WFOMC, to prove domain-liftaibility of FO$^2$ extended with DAG axioms. For expanding our results to cardinality constraints and counting quantifiers, we exploit the results from \cite{kuzelka2020weighted}. Whereas, in  order to show domain liftaibility of the proposed (recursion-based) counting formula, we provide a bottom-up algorithm, which is similar to the algorithm provided in \cite{LinearOrder}.
  
  

%%% mode: latex
%%% TeX-master: "main"
%%% End:

